An Algorithmic Pipeline for Analyzing Multi-parametric Flow Cytometry Data

Flow cytometry (FC) is a single-cell profiling platform for measuring the phenotypes of individual cells from millions of cells in biological samples. FC employs high-throughput technologies and generates high-dimensional data, and hence algorithms for analyzing the data represent a bottleneck. This dissertation addresses several computational challenges arising in modern cytometry while mining information from high-dimensional and high-content biological data. A collection of combinatorial and statistical algorithms for locating, matching, prototyping, and classifying cellular populations from multi-parametric FC data is developed. The algorithmic pipeline, flowMatch, developed in this dissertation consists of five well-defined algorithmic modules to (1) transform data to stabilize within-population variance, (2) identify cell populations by robust clustering algorithms, (3) register cell populations across samples, (4) encapsulate a class of samples with templates, and (5) classify samples based on their similarity with the templates. Components of flowMatch can work independently or collaborate with each other to perform the complete data analysis. flowMatch is made available as an open-source R package in Bioconductor. We have employed flowMatch for classifying leukemia samples, evaluating the phosphorylation effects on T cells, classifying healthy immune profiles, and classifying the vaccination status of HIV patients. In these analyses, the pipeline is able to reach biologically meaningful conclusions quickly and efficiently with the automated algorithms. The algorithms included in flowMatch can also be applied to problems outside of flow cytometry such as in microarray data analysis and image recognition. Therefore, this dissertation contributes to the solution of fundamental problems in computational cytometry and related domains.

==> mydefs.tex <==
%
%  mydefs.tex  2007-03-19  Mark Senn  http://www.ecn.purdue.edu/~mark
%
%  Command definitions that can be used in all documents that have
%      \input{mydefs}
%

% CHANGE NEXT 3 LINES?
% Define \be and \ee to start and end the equation environment.
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}

% CHANGE NEXT 12 LINES?
% Define \Repeat so, for example,
%     \Repeat{whatever}{10}
% is the same as typing whatever 10 times.
\newcount{\myi}
\newcommand{\Repeat}[2]{%
    \myi=0
    \loop
        \ifnum\myi<#2
        #1
        \advance\myi by 1
    \repeat
}

% CHANGE NEXT 3 LINES?
% Make "\Sum ab" or "\Sum{a}{b}" do "\sum_{a}^{b}".
% This can only be used when in math mode.
\newcommand\Sum[2]{\sum_{#1}^{#2}}

% CHANGE NEXT 4 LINES?
% Make "\xn" do "$x_n$".
% Because this definition contains the "$" to go into math mode
% this definition must be used when not in math mode.
\newcommand{\xn}{$x_n$}

% CHANGE NEXT 5 LINES?
% Since \xn is already defined we must use \renewcommand to redefine it.
% Normally you would not have the above definition for \xn in this file
% if you were just going to override it later.
% The \ensuremath goes into math mode if not already in math mode.
\renewcommand{\xn}{\ensuremath{x_n}}



==> summary.tex <==
%
%  summary.tex  2007-02-06  Mark Senn  http://www.ecn.purdue.edu/~mark
%

\chapter{Summary}

This is the summary chapter.

